MResT: Multi-Resolution Sensing for Real-Time Control with Vision-Language Models

Leveraging sensing modalities across diverse spatial and temporal resolutions can improve performance of robotic manipulation tasks. Multi-spatial resolution sensing provides hierarchical information captured at different spatial scales and enables both coarse and precise motions. Simultaneously multi-temporal resolution sensing enables the agent to exhibit high reactivity and real-time control. In this work, we propose a framework, MResT (Multi-Resolution Transformer), for learning generalizable language-conditioned multi-task policies that utilize sensing at different spatial and temporal resolutions using networks of varying capacities to effectively perform real time control of precise and reactive tasks. We leverage off-the-shelf pretrained vision-language models to operate on low-frequency global features along with small non-pretrained models to adapt to high frequency local feedback. Through extensive experiments in 3 domains (coarse, precise and dynamic manipulation tasks), we show that our approach significantly improves (2X on average) over recent multi-task baselines. Further, our approach generalizes well to visual and geometric variations in target objects and to varying interaction forces.

==> abstract_old.tex <==
TODO (DON'T READ)
For spatial precision tasks, robots require in-hand cameras and force feedback for better localization.
For generalization, we need large vision-language models.
However, large VLMs (VFMs) have certain disadvantages: First, they have slow inference which makes them unusable for real-time control.
Second, to enable VFMs to solve novel out-of-domain manipulation tasks they may need finetuning, which can lead to a loss of robustness.
%low-level visual details (e.g. edges for insertion) we need to finetune them, but such finetuning loses robustness.
We address these challenges by proposing a multi-resolution multi-modal language-conditioned policy which conditions on multiple views and force-feedback. 
This multi-modal policy uses static third person views for coarse localization while utilizing smaller and faster networks for in-hand cameras and force-torque data.
To enable real-time control, we incorporate different sensor modalities at different frequencies. We use large VLMs with slow inference at a lower frequency while smaller networks with fast inference at higher frequencies.
Further, our low-frequency VFMs operate on static views to extract coarse visual features while we use high frequency models on eye-in-hand camera views and force-torque data for fine-grained feedback. 
This allows us to utilize the robustness of VFMs  while learning a robust closed-loop visuomotor policy.


==> intro_old.tex <==
Using multiple spatial modalities can also enable generalization by utilizing global information such as third-person camera images for course localization of the target object but using the local information from in-hand cameras (object edges) and force-torque feedback for low level control. Learning generalizable policies for robotic manipulation tasks is a problem addressed by a lot of prior work especially in the context of multi-task learning. In this work, we focus on multi-task learning using multiple sensing modalities at different spatio-temporal resolutions. Towards such generalizable multi-task settings, recent works have shown the benefits of using large pretrained vision or vision-language models (VLMs) \cite{shridhar2022cliport, moo2023arxiv, jiang2022vima}.
Given that these large VLMs are often trained on large-scale (e.g. internet scale) general purpose 
data, they show impressive zero-shot generalization capabilities \cite{radford2021learning, li2021align, alayrac2022flamingo, jia2021scaling}.
However, such large VLMs often have certain disadvantages. 
First, given their large size (e.g. Flamingo has 80B parameters \cite{alayrac2022flamingo}), 
they have slow inference which makes them unusable for real-time closed-loop control which is necessary for reactive tasks. Such approaches do not address the utility of using multiple sensing modalities at different spatial and temporal resolutions.
Second, since VLMs are often trained on out-of-domain data using them to solve novel in-domain manipulation tasks may require finetuning \cite{sharmalossless}.
However, task-specific finetuning can lead to a loss of robustness and reduced generalization abilities.




Real-world reactive and precise robotic tasks often necessitate agents to employ sensing techniques at multiple spatial scales, encompassing both global and local information.
For instance, in an insertion task, the robot globally localizes the object, approaches it, utilizes in-hand cameras for finer motions,
and reacts to force-feedback for task completion. 
In this work, we focus on such precise and reactive manipulation tasks.
However, instead of learning such tasks in single-task settings we aim to learn generalizable reactive skills for such task domains. Learning in language conditioned multi-task settings allows for data sharing, e.g., recognizing common task structures, which can significantly benefit overall task performance and importantly enable task generalization.  

\begin{enumerate}
    \item 1-2 line, some people freeze, others finetune, we use advantages of both in our multi-modal framework.
\end{enumerate}



Towards such generalizable multi-task settings, recent works have shown the benefits of using large pretrained vision or vision-language models (VLMs) \cite{shridhar2022cliport, moo2023arxiv, jiang2022vima}.
Given that these large VLMs are often trained on large-scale (e.g. internet scale) general purpose 
data, they show impressive zero-shot generalization capabilities \cite{radford2021learning, li2021align, alayrac2022flamingo, jia2021scaling}.
However, such large VLMs often have certain disadvantages. 
First, given their large size (e.g. Flamingo has 80B parameters \cite{alayrac2022flamingo}), 
they have slow inference which makes them unusable for real-time closed-loop control which is necessary for reactive tasks. Such approaches do not address the utility of using multiple sensing modalities at different spatial and temporal resolutions.
Second, since VLMs are often trained on out-of-domain data using them to solve novel in-domain manipulation tasks may require finetuning \cite{sharmalossless}.
However, task-specific finetuning can lead to a loss of robustness and reduced generalization abilities.

\textcolor{ms_red}{
In this work, we focus on learning generalizable multi-task policies using reactive and precise manipulation tasks.
Prior works within robot manipulation often only use VLMs for task-specification and not to learn generalizable policies. While other works that show generalization only use templated open-loop primitives. 
By contrast, to these works we focus on ....
}


To our work, we aim to address the above challenges by proposing a multi-resolution multi-modal policy learning approach.
Our policy uses sensing modalities at different spatial resolutions, camera views (static third person view and first-person eye-in-hand view) along with proprioception and force-torque feedback as inputs.
Using multiple sensing modalities benefits contact-rich precise manipulation by leveraging static third person views for coarse localization while eye-in-hand and force-torque feedback are leveraged for fine-grained motions.
To enable real-time control we incorporate different modalities at different frequencies. We use large VLMs with slow inference at a lower frequency while smaller networks provide fast inference at higher frequencies.
Our low-frequency VLMs operate on static views to extract coarse visual features while we use high frequency models on eye-in-hand camera views and force-torque data for fine-grained feedback. 

Additionally, we learn novel in-domain reactive manipulation tasks using pretrained VLMs without sacrificing their generalization abilities. To achieve this, we propose a novel network architecture that combines a pretrained large \textbf{frozen} model with a trained-from-scratch smaller FiLM based model.
Freezing the pretrained model maintains its generalization abilities while finetuning the smaller model allows the agent to successfully learn reactive manipulation tasks.
Further, as noted above, we use the large frozen VLM at a lower frequency to extract semantic and coarse spatial features from third person camera views.
While we use the finetuned smaller model at a higher frequency to  extract task-specific fine-grained features.

